A Walk in Facebook: Uniform Sampling of Users in Online Social Networks

Our goal in this paper is to develop a practical framework for obtaining a uniform sample of users in an online social network (OSN) by crawling its social graph. Such a sample allows to estimate any user property and some topological properties as well. To this end, first, we consider and compare several candidate crawling techniques. Two approaches that can produce approximately uniform samples are the Metropolis-Hasting random walk (MHRW) and a re-weighted random walk (RWRW). Both have pros and cons, which we demonstrate through a comparison to each other as well as to the "ground truth." In contrast, using Breadth-First-Search (BFS) or an unadjusted Random Walk (RW) leads to substantially biased results. Second, and in addition to offline performance assessment, we introduce online formal convergence diagnostics to assess sample quality during the data collection process. We show how these diagnostics can be used to effectively determine when a random walk sample is of adequate size and quality. Third, as a case study, we apply the above methods to Facebook and we collect the first, to the best of our knowledge, representative sample of Facebook users. We make it publicly available and employ it to characterize several key properties of Facebook.

==> bios.tex <==
%

\vspace{-30pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/Minas_photo.eps}}]
{Minas Gjoka} received his B.S. (2005) degree in Computer Science  at the Athens
University of Economics and Business, Greece, and his M.S. (2008) and Ph.D. (2010) degrees in Networked Systems at the University of California, Irvine. He is currently a postdoc at the University of California, Irvine. His research  interests are in the general areas of networking and distributed 
systems, with emphasis on online social networks, peer-to-peer systems,  and network measurement.
\end{IEEEbiography}

\vspace{-30pt}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/Kurant_bio.eps}}]
%
{Maciej Kurant} received a M.Sc. degree from Gdansk University of Technology, Poland, in 2002, and a Ph.D. degree from EPFL, Lausanne, Switzerland, in 2009. Currently, he is a postdoc at University of California, Irvine. His main areas of research interest include sampling and inference from large-scale networks (such
as Internet topologies or the human brain), multipath routing with FEC, and survivability in WDM networks. He is also a founder of AcronymCreator.net - a tool that helps creating new, meaningful acronyms.
\end{IEEEbiography}
\vspace{-30pt}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/Butts_photo.eps}}]
{Carter T. Butts} received his B.S. degree from Duke University in 1996, and his Ph.D. from Carnegie Mellon University in 2002.  In 2002 he joined the Department of Sociology at the University of California, Irvine, where he is currently associate professor; he holds appointments in the Departments of Sociology and Statistics, and is a member of the Institute for Mathematical Behavioral Sciences and the California Institute for Telecommunications and Information Technology.  He currently serves as an area editor for Computational and Mathematical Organization Theory, and serves on the editorial boards of the Journal of Mathematical Sociology and Sociological Methodology.   He holds several paper awards from the American Sociological Association, was the 2010 recipient of the Leo A. Goodman early career award from the ASA Section on Methodology, and was the 2008 recipient of the Linton C. Freeman Award from the International Network for Social Network Analysis.  His current research interests include the structure of spatially embedded large-scale interpersonal networks; models for informant accuracy, network inference, and graph comparison; representation and modeling of intertemporal relational data; and measurement and modeling of online social networks.
\end{IEEEbiography}
\vspace{-10pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/athina.eps}}]
{Athina Markopoulou} (SM '98, M'02) is an assistant professor in the EECS Dept. at the University of California, Irvine. She received the Diploma degree in Electrical and Computer Engineering from the National Technical University of Athens, Greece, in 1996, and the M.S. and Ph.D. degrees, both in Electrical Engineering, from Stanford University in 1998 and 2003, respectively. She has been a postdoctoral fellow at Sprint Labs (2003) and at Stanford University (2004-2005), and a member of the technical staff at Arastra Inc. (2005). Her research interests include network coding, network measurements and security, media streaming and online social networks. She received the NSF CAREER award in 2008.
\end{IEEEbiography}

\vspace{-10pt}

==> diagnostics.tex <==

\label{sec:diagnostics}

%

Convergence is defined as the point in which the sample has reached the stationary distribution. We refer to the collection of tools used for convergence assessment as convergence diagnostics. We would like to use such diagnostics to answer questions such as: i) how many iterations are needed before we declare convergence? ii) how many of the initial elements in each sequence do we need to discard?

Given that we do not have knowledge of the target distribution, we can only estimate convergence from the statistical properties of the sequences as they are collected. 
%
Here we present two such convergence diagnostics, Geweke and Gelman-Rubin which we will later use with various user node properties.

\textbf{{\em Geweke} } The Geweke diagnostic \cite{geweke} tests the null hypothesis that a single Markov chain is in the stationary distribution and produces a z-statistic for each estimated parameter by comparing the mean and variance of segments from the beginning and end of a single  sequence : $z = \frac{\bar \theta_{A} - \bar \theta_{W} }{\sqrt{ Var(\theta_{A}) - Var(\theta_{W}) } } $  ,  where A is the first interval and W the last interval. Similarity in the z-scores
 %
 of these two segments provides evidence for convergence. 

%
%
%
%
%
%


\textbf{{\em Gelman-Rubin} }  The Gelman and Rubin diagnostic \cite{gelman-rubin}  monitors convergence of the output of a MCMC process with $m$ multiple sequences whose starting points are overdispersed in the target distribution. It indicates convergence when the output from all sequences is similar. The Gelman-Rubin diagnostic is applied to a single scalar parameter in the sequences and it is based on a comparison of within-sequence and between-sequence variances.  More specifically, the variance of the stationary distribution is estimated in two ways different ways: i) the empirical variance from all sequences combined, defined as V, using both between-sequence and within-sequence information. ii) the mean of all empirical variances within each sequence, defined as  W.  If all $m$ sequences  have converged, then both these estimates of variance converge to the same value and the Gelman-Rubin diagnostic R reaches the value 1. Otherwise the variance of the estimate V over all sequences is expected to be higher because of the selection of overdispersed starting points while the variance of the within-sequence estimate W is expected to be lower, since the individual sequences have not mixed enough.


%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

%
